Towards dense volumetric pancreas segmentation in CT using 3D fully convolutional networks

Pancreas segmentation in computed tomography imaging has been historically difficult for automated methods because of the large shape and size variations between patients. In this work, we describe a custom-build 3D fully convolutional network (FCN) that can process a 3D image including the whole pancreas and produce an automatic segmentation. We investigate two variations of the 3D FCN architecture; one with concatenation and one with summation skip connections to the decoder part of the network. We evaluate our methods on a dataset from a clinical trial with gastric cancer patients, including 147 contrast enhanced abdominal CT scans acquired in the portal venous phase. Using the summation architecture, we achieve an average Dice score of 89.7 $\pm$ 3.8 (range [79.8, 94.8]) % in testing, achieving the new state-of-the-art performance in pancreas segmentation on this dataset.

==> _spie2018_references.tex <==
@inproceedings{lee2015evaluation,
	title={Evaluation of five image registration tools for abdominal CT: pitfalls and opportunities with soft anatomy},
	author={Lee, Christopher P and Xu, Zhoubing and Burke, Ryan P and Baucom, Rebeccah B and Poulose, Benjamin K and Abramson, Richard G and Landman, Bennett A},
	booktitle={Proceedings of SPIE--the International Society for Optical Engineering},
	volume={9413},
	year={2015},
	organization={NIH Public Access}
}

@article{roth2017spatial,
  title={Spatial Aggregation of Holistically-Nested Convolutional Neural Networks for Automated Pancreas Localization and Segmentation},
  author={Roth, Holger R and Lu, Le and Lay, Nathan and Harrison, Adam P and Farag, Amal and Sohn, Andrew and Summers, Ronald M},
  journal={arXiv preprint arXiv:1702.00045},
  year={2017}
}

@inproceedings{long2015fully,
  title={Fully convolutional networks for semantic segmentation},
  author={Long, Jonathan and Shelhamer, Evan and Darrell, Trevor},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3431--3440},
  year={2015}
}

@article{zhou2016pancreas,
  title={Pancreas Segmentation in Abdominal CT Scan: A Coarse-to-Fine Approach},
  author={Zhou, Yuyin and Xie, Lingxi and Shen, Wei and Fishman, Elliot and Yuille, Alan},
  journal={arXiv preprint arXiv:1612.08230},
  year={2016}
}

@article{roth2017hierarchical,
  title={Hierarchical {3D} fully convolutional networks for multi-organ segmentation},
  author={Roth, Holger R and Oda, Hirohisa and Hayashi, Yuichiro and Oda, Masahiro and Shimizu, Natsuki and Fujiwara, Michitaka and Misawa, Kazunari and Mori, Kensaku},
  journal={arXiv preprint arXiv:1704.06382},
  year={2017}
}

@inproceedings{cciccek20163d,
  title={{3D} U-Net: learning dense volumetric segmentation from sparse annotation},
  author={{\c{C}}i{\c{c}}ek, {\"O}zg{\"u}n and Abdulkadir, Ahmed and Lienkamp, Soeren S and Brox, Thomas and Ronneberger, Olaf},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={424--432},
  year={2016},
  organization={Springer}
}

@inproceedings{drozdzal2016importance,
  title={The importance of skip connections in biomedical image segmentation},
  author={Drozdzal, Michal and Vorontsov, Eugene and Chartrand, Gabriel and Kadoury, Samuel and Pal, Chris},
  booktitle={International Workshop on Large-Scale Annotation of Biomedical Data and Expert Label Synthesis},
  pages={179--187},
  year={2016},
  organization={Springer}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@inproceedings{milletari2016v,
  title={V-net: Fully convolutional neural networks for volumetric medical image segmentation},
  author={Milletari, Fausto and Navab, Nassir and Ahmadi, Seyed-Ahmad},
  booktitle={{3D} Vision ({3DV}), 2016 Fourth International Conference on},
  pages={565--571},
  year={2016},
  organization={IEEE}
}

@inproceedings{oda2016regression,
  title={Regression forest-based atlas localization and direction specific atlas generation for pancreas segmentation},
  author={Oda, Masahiro and Shimizu, Natsuki and Karasawa, Ken’ichi and Nimura, Yukitaka and Kitasaka, Takayuki and Misawa, Kazunari and Fujiwara, Michitaka and Rueckert, Daniel and Mori, Kensaku},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={556--563},
  year={2016},
  organization={Springer}
}


@article{cerrolaza2015automatic,
	title={Automatic multi-resolution shape modeling of multi-organ structures},
	author={Cerrolaza, Juan J and Reyes, Mauricio and Summers, Ronald M and Gonz{\'a}lez-Ballester, Miguel {\'A}ngel and Linguraru, Marius George},
	journal={Medical image analysis},
	volume={25},
	number={1},
	pages={11--21},
	year={2015},
	publisher={Elsevier}
}

@article{okada2015abdominal,
	title={Abdominal multi-organ segmentation from CT images using conditional shape--location and unsupervised intensity priors},
	author={Okada, Toshiyuki and Linguraru, Marius George and Hori, Masatoshi and Summers, Ronald M and Tomiyama, Noriyuki and Sato, Yoshinobu},
	journal={Medical image analysis},
	volume={26},
	number={1},
	pages={1--18},
	year={2015},
	publisher={Elsevier}
}

@inproceedings{wang2013multi,
	title={Multi-atlas segmentation with robust label transfer and label fusion},
	author={Wang, Hongzhi and Pouch, Alison and Takabe, Manabu and Jackson, Benjamin and Gorman, Joseph and Gorman, Robert and Yushkevich, Paul A},
	booktitle={Information processing in medical imaging: proceedings of the... conference},
	volume={23},
	pages={548},
	year={2013},
	organization={NIH Public Access}
}

@article{iglesias2015multi,
	title={Multi-atlas segmentation of biomedical images: a survey},
	author={Iglesias, Juan Eugenio and Sabuncu, Mert R},
	journal={Medical image analysis},
	volume={24},
	number={1},
	pages={205--219},
	year={2015},
	publisher={Elsevier}
}

@article{rohlfing2004evaluation,
	title={Evaluation of atlas selection strategies for atlas-based image segmentation with application to confocal microscopy images of bee brains},
	author={Rohlfing, Torsten and Brandt, Robert and Menzel, Randolf and Maurer, Calvin R},
	journal={NeuroImage},
	volume={21},
	number={4},
	pages={1428--1442},
	year={2004},
	publisher={Elsevier}
}

@article{wolz2013automated,
	title={Automated abdominal multi-organ segmentation with subject-specific atlas generation},
	author={Wolz, Robin and Chu, Chengwen and Misawa, Kazunari and Fujiwara, Michitaka and Mori, Kensaku and Rueckert, Daniel},
	journal={IEEE Transactions on Medical Imaging},
	volume={32},
	number={9},
	pages={1723--1730},
	year={2013},
	publisher={IEEE}
}


@article{tong2015discriminative,
	title={Discriminative dictionary learning for abdominal multi-organ segmentation},
	author={Tong, Tong and Wolz, Robin and Wang, Zehan and Gao, Qinquan and Misawa, Kazunari and Fujiwara, Michitaka and Mori, Kensaku and Hajnal, Joseph V and Rueckert, Daniel},
	journal={Medical Image Analysis},
	volume={23},
	number={1},
	pages={92--104},
	year={2015},
	publisher={Elsevier}
}

@inproceedings{christ2016automatic,
	title={Automatic Liver and Lesion Segmentation in CT Using Cascaded Fully Convolutional Neural Networks and {3D} Conditional Random Fields},
	author={Christ, Patrick Ferdinand and Elshaer, Mohamed Ezzeldin A and Ettlinger, Florian and Tatavarty, Sunil and Bickel, Marc and Bilic, Patrick and Rempfler, Markus and Armbruster, Marco and Hofmann, Felix and D’Anastasi, Melvin and others},
	booktitle={MICCAI},
	pages={415--423},
	year={2016},
	organization={Springer}
}

@inproceedings{zhou2016three,
	title={Three-Dimensional CT Image Segmentation by Combining {2D} Fully Convolutional Network with {3D} Majority Voting},
	author={Zhou, Xiangrong and Ito, Takaaki and Takayama, Ryosuke and Wang, Song and Hara, Takeshi and Fujita, Hiroshi},
	booktitle={LABELS workshop},
	pages={111--120},
	year={2016},
	organization={Springer}
}


@inproceedings{roth2016spatial,
	title={Spatial aggregation of holistically-nested networks for automated pancreas segmentation},
	author={Roth, Holger R and Lu, Le and Farag, Amal and Sohn, Andrew and Summers, Ronald M},
	booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
	pages={451--459},
	year={2016},
	organization={Springer}
}


@inproceedings{roth2015deeporgan,
	title={Deeporgan: Multi-level deep convolutional networks for automated pancreas segmentation},
	author={Roth, Holger R and Lu, Le and Farag, Amal and Shin, Hoo-Chang and Liu, Jiamin and Turkbey, Evrim B and Summers, Ronald M},
	booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
	pages={556--564},
	year={2015},
	organization={Springer}
}


@article{hu2017automatic,
	title={Automatic abdominal multi-organ segmentation using deep convolutional neural network and time-implicit level sets},
	author={Hu, Peijun and Wu, Fa and Peng, Jialin and Bao, Yuanyuan and Chen, Feng and Kong, Dexing},
	journal={International journal of computer assisted radiology and surgery},
	volume={12},
	number={3},
	pages={399--411},
	year={2017},
	publisher={Springer}
}

@inproceedings{gibson2017towards,
	title={Towards Image-Guided Pancreas and Biliary Endoscopy: Automatic Multi-organ Segmentation on Abdominal CT with Dense Dilated Networks},
	author={Gibson, Eli and Giganti, Francesco and Hu, Yipeng and Bonmati, Ester and Bandula, Steve and Gurusamy, Kurinchi and Davidson, Brian R and Pereira, Stephen P and Clarkson, Matthew J and Barratt, Dean C},
	booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
	pages={728--736},
	year={2017},
	organization={Springer}
}

@article{dou20173d,
	title={3D deeply supervised network for automated segmentation of volumetric medical images},
	author={Dou, Qi and Yu, Lequan and Chen, Hao and Jin, Yueming and Yang, Xin and Qin, Jing and Heng, Pheng-Ann},
	journal={Medical Image Analysis},
	year={2017},
	publisher={Elsevier}
}

@inproceedings{prasoon2013deep,
	title={Deep feature learning for knee cartilage segmentation using a triplanar convolutional neural network},
	author={Prasoon, Adhish and Petersen, Kersten and Igel, Christian and Lauze, Fran{\c{c}}ois and Dam, Erik and Nielsen, Mads},
	booktitle={International conference on medical image computing and computer-assisted intervention},
	pages={246--253},
	year={2013},
	organization={Springer}
}

@article{kamnitsas2017efficient,
	title={Efficient multi-scale 3D CNN with fully connected CRF for accurate brain lesion segmentation},
	author={Kamnitsas, Konstantinos and Ledig, Christian and Newcombe, Virginia FJ and Simpson, Joanna P and Kane, Andrew D and Menon, David K and Rueckert, Daniel and Glocker, Ben},
	journal={Medical image analysis},
	volume={36},
	pages={61--78},
	year={2017},
	publisher={Elsevier}
}

@article{lecun2015deep,
	title={Deep learning},
	author={LeCun, Yann and Bengio, Yoshua and Hinton, Geoffrey},
	journal={Nature},
	volume={521},
	number={7553},
	pages={436--444},
	year={2015},
	publisher={Nature Research}
}



@article{chen2016voxresnet,
title={VoxResNet: Deep Voxelwise Residual Networks for Volumetric Brain Segmentation},
author={Chen, Hao and Dou, Qi and Yu, Lequan and Heng, Pheng-Ann},
journal={arXiv preprint arXiv:1608.05895},
year={2016}
}


